A Big Data-empowered System for Real-time Detection of Regional Discriminatory Comments on Vietnamese Social Media

Regional discrimination is a persistent social issue in Vietnam. While existing research has explored hate speech in the Vietnamese language, the specific issue of regional discrimination remains under-addressed. Previous studies primarily focused on model development without considering practical system implementation. In this work, we propose a task called Detection of Regional Discriminatory Comments on Vietnamese Social Media, leveraging the power of machine learning and transfer learning models. We have built the ViRDC (Vietnamese Regional Discrimination Comments) dataset, which contains comments from social media platforms, providing a valuable resource for further research and development. Our approach integrates streaming capabilities to process real-time data from social media networks, ensuring the system's scalability and responsiveness. We developed the system on the Apache Spark framework to efficiently handle increasing data inputs during streaming. Our system offers a comprehensive solution for the real-time detection of regional discrimination in Vietnam.

==> section7_limitation.tex <==
\section{Limitation}

Một trong những hạn chế chính của nghiên cứu này là khả năng tối ưu hóa tham số của mô hình bị giới hạn bởi phần cứng. Do hạn chế về tài nguyên tính toán, chúng tôi không thể thực hiện các phương pháp tối ưu hóa tham số toàn diện cho các mô hình học sâu O. Điều này có thể dẫn đến việc mô hình không đạt được hiệu suất tối ưu nhất. 

Ngoài ra, bộ dữ liệu sử dụng trong nghiên cứu có dấu hiệu không cần bằng về các đặc trưng. Cụ thể, các đặc trưng trong bộ dữ liệu có thể không đại diện đầy đủ cho toàn bộ các hình thức định kiến và phân biệt đối với các khu vực, cụ thể là những từ ngữ phân biệt ở các vùng miền tiêu biểu lớn (các miền bắc, trung, nam) ở đất nước Việt Nam mà chứa các số lượng nhỏ các bình luận phân biệt các tỉnh thành nhỏ lẻ khác , dẫn đến việc mô hình có thể hoạt động kém hiệu quả khi áp dụng vào các tình huống thực tế khác biệt. Điều này có thể ảnh hưởng đến độ tin cậy và khả năng tổng quát hóa của các kết quả nghiên cứu. 

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


